Ekya: Continuous Learning of Video Analytics Models on Edge Compute Servers

Video analytics applications use edge compute servers for the analytics of the videos (for bandwidth and privacy). Compressed models that are deployed on the edge servers for inference suffer from data drift, where the live video data diverges from the training data. Continuous learning handles data drift by periodically retraining the models on new data. Our work addresses the challenge of jointly supporting inference and retraining tasks on edge servers, which requires navigating the fundamental tradeoff between the retrained model's accuracy and the inference accuracy. Our solution Ekya balances this tradeoff across multiple models and uses a micro-profiler to identify the models that will benefit the most by retraining. Ekya's accuracy gain compared to a baseline scheduler is 29% higher, and the baseline requires 4x more GPU resources to achieve the same accuracy as Ekya.

==> backups/algo_thiefsched_0916.tex <==
% \begin{algorithm}
%  \KwData{Configuration profiles $\Gamma_v$ and $\Lambda_v$ and resource allocations $g^{c}_R$ and $g^{c}_I$ for video $v$}
%  \KwResult{The optimal configurations $\gamma^{opt}_{v}$ and  $\lambda^{opt}_{v}$}
%  
%  best\_accuracy = 0\;
%  \For{$\lambda_v$ in $\Lambda_v$}{
%     \For{$\gamma_v$ in $\Gamma_v$}{
%          accuracy = simulator([$\lambda_v$, $\gamma_v$], [$g^{c}_R$, $g^{c}_I$])\;
%         \If{accuracy > best\_accuracy}{
%             $\lambda^{opt}_{v}$, $\gamma^{opt}_{v}$ = $\lambda_v$, $\gamma_v$\;
%             best\_accuracy = accuracy\;
%         }
%     }
%  }
% 
% return $\lambda^{opt}_{v}$, $\gamma^{opt}_{v}$\;
% \caption{ConfigurationPickingRoutine}
% \label{algo:config_pick}
%\end{algorithm}

\begin{algorithm}[t]
\small
 \KwData{Training ($\Gamma$) and inference ($\Lambda$) configurations}
 \KwResult{GPU allocations $\mathcal{R}$ and $\mathcal{I}$, chosen configurations ($\gamma \in \Gamma$, $\lambda \in \Lambda$) $\forall v \in V$}% for the period T.}
 
 % Run in a loop to do iterations of configuration selection and resource allocation
all\_jobs[] = Union of inference and training jobs of videos $V$\;
\tcc{Initialize with fair allocation}
 best\_alloc[] = fair\_allocation(all\_jobs)\; 
% \For{iteration in iteration\_count}{
     % Perform SCO - Single camera optimization which picks the best hyperparameters.
%     \For{v in V}{
%        v.training\_config = {\sf\footnotesize PickConfigurations}(v, curr\_alloc[v]) \;
%     }
 best\_accuracy\_avg =  {\sf\footnotesize PickConfigurations}(best\_alloc, {\bf out} best\_configs[]) \;
     % Perform thief resource stealing
     \tcc{Thief resource stealing}
%     best\_accuracy\_avg = 0\;
     \For{\text{\em thief\_job} in \text{\em all\_jobs[]}}{
        \For{\text{\em victim\_job} in \text{\em all\_jobs[]}}{
            \If{\text{\em thief\_job} == \text{\em victim\_job}} {\bf continue\;}
            temp\_alloc[] $\leftarrow$ best\_alloc[]\;
            \While{true}{
                \tcc{$\Delta$ is the increment of stealing}
                temp\_alloc[victim\_job] $-$= $\Delta$\;
                temp\_alloc[thief\_job] $+$= $\Delta$\;
                \If{{\em temp\_alloc[victim\_job]} < {\em 0}}{
                    \bf break\;
                }
                \tcc{Calculate accuracy over retraining window and pick configurations.}accuracy\_avg = {\sf\footnotesize PickConfigurations}(temp\_alloc, {\bf out} temp\_configs[])\;
                %\tcc{Calculate accuracy over retraining window and pick configurations.}%accuracy\_$\alpha$ = {\sf\footnotesize Estim}(temp\_configs[], temp\_alloc[])\;
                \If{{\em accuracy\_avg} > {\em best\_accuracy\_avg}}{
                    best\_alloc[] = temp\_alloc[]\;
                    best\_accuracy\_avg = accuracy\_avg\;
                    best\_configs[] = temp\_configs[];
                }
                \Else{\bf break\;}
            }
        }
     }
% }
 {\bf return} {best\_alloc[], best\_configs[]}\;
 
 \caption{Thief Scheduler.
 %\junchen{it's going through all the users, rather than iterative algorithm.. may need a better structure}
 %\romil{Explain estim in function call.}
 }
 \label{algo:thief_sched}
\end{algorithm}

% PickConfigurations
% For the given allocation, finds the best configuration and returns the accuracy gotten by the best configuration and given resource allocation.

\begin{algorithm}[t]
\small
 \KwData{Initial resource allocations $\mathcal{R}^\prime$ and $\mathcal{I}^\prime$ and configurations ($\Lambda$)}
 \KwResult{GPU allocations $\mathcal{R}$ and $\mathcal{I}$, chosen configurations ($\gamma \in \Gamma$, $\lambda \in \Lambda$) $\forall v \in V$}% for the period T.}
 
 % Run in a loop to do iterations of configuration selection and resource allocation
all\_jobs[] = Union of inference and training jobs of videos $V$\;
\tcc{Initialize with fair allocation}
 best\_alloc[] = fair\_allocation(all\_jobs)\; 
% \For{iteration in iteration\_count}{
     % Perform SCO - Single camera optimization which picks the best hyperparameters.
%     \For{v in V}{
%        v.training\_config = {\sf\footnotesize PickConfigurations}(v, curr\_alloc[v]) \;
%     }
 best\_accuracy\_avg =  {\sf\footnotesize PickConfigurations}(best\_alloc, {\bf out} best\_configs[]) \;
     % Perform thief resource stealing
     \tcc{Thief resource stealing}
%     best\_accuracy\_avg = 0\;
     \For{\text{\em thief\_job} in \text{\em all\_jobs[]}}{
        \For{\text{\em victim\_job} in \text{\em all\_jobs[]}}{
            \If{\text{\em thief\_job} == \text{\em victim\_job}} {\bf continue\;}
            temp\_alloc[] $\leftarrow$ best\_alloc[]\;
            \While{true}{
                \tcc{$\Delta$ is the increment of stealing}
                temp\_alloc[victim\_job] $-$= $\Delta$\;
                temp\_alloc[thief\_job] $+$= $\Delta$\;
                \tcc{Calculate accuracy over retraining window and pick configurations.}accuracy\_avg = {\sf\footnotesize PickConfigurations}(temp\_alloc, {\bf out} temp\_configs[])\;
                %\tcc{Calculate accuracy over retraining window and pick configurations.}%accuracy\_$\alpha$ = {\sf\footnotesize Estim}(temp\_configs[], temp\_alloc[])\;
                \If{{\em accuracy\_avg} > {\em best\_accuracy\_avg}}{
                    best\_alloc[] = temp\_alloc[]\;
                    best\_accuracy\_avg = accuracy\_avg\;
                    best\_configs[] = temp\_configs[];
                }
                \Else{\bf break\;}
            }
        }
     }
% }
 {\bf return} {best\_alloc[], best\_configs[]}\;
 
 \caption{PickConfigurations \romil{FORMAT LATER}
 }
 \label{algo:pickconfigs}
\end{algorithm}


==> eval-new.tex <==
\section{Evaluation}
\label{sec:evaluation}

We evaluate \name{} on the Waymo and Cityscapes data. %The highlights are:

\begin{itemize}
    \item With multiple cameras sharing the resources on an edge server, \name{} achieves upto \romilc{16}\% \romil{This is sim, check exact with zhengxu} points higher accuracy than the fair sharing baseline. Attaining the same accuracy with a fair-sharing scheduler would require upto \romilc{$2.xx\times$} more resources.
    \item With the same resource provisioning, \name{} is able to support upto $5\times$ more video streams than the fair scheduler.
    \item \name{}'s performance gracefully degrades with reduction in resources to the baseline that does not retrain since it evaluates the cost of retraining on the accuracy. 
\end{itemize}

\subsection{Methodology}
\label{subsec:eval-setup}

\junchen{need to update}

\noindent\textbf{Datasets.} For our evaluation, we use the Waymo Open\cite{waymo} and Cityscapes\cite{cityscapes} datasets, two popular video datasets containing dashboard camera footage of cars driving through cities in the US and Europe. Cityscapes has frames from 27 video streams training with a total of 5000 pixel-level annotated frames, while Waymo Open has 1000 video segments with a total of 200000 frames.

The workload in Cityscapes is constructed by treating each city's video as an independent video stream feeding into {\name} for inference and retraining. The workload in Waymo Open is constructed by creating video streams by concatenating 20s-video segments belonging to the same city in chronological order. Each video stream in both datasets is then split into 10 retraining windows. These workloads are representative of independent video-streams with local variations which necessitate retraining for their specific data-distributions.



% \noindent\textbf{System Implementation.}\junchen{shrink or remove given the impl section}
% We implement a prototype of \name in Python using Ray\cite{ray} for asynchronous operations and RPCs. 
% Each video stream is modelled as an independent Ray actor whose resource allocation for inference and training is periodically updated by the Ekya master.

% % Write about microprofiling
% %\mypara{Microprofiling}
% The Ekya implementation ingests video streams and splits it into evenly sized retraining periods. At the start of each retraining period, the hyperparameters are micro-profiled \ref{sec:microprofiling} and the thief scheduler is run to compute the resource allocations for training and inference jobs. 
% %This resource allocation is then enforced by Ekya by launching new training processes and restarting the inference processes with updated resource weights. 

% Ekya requires fine-grained GPU allocation between inference and training processes. 
% Talk about memory isolation in Ekya.
% Talk about nvidia MPS resource sharing



\noindent\textbf{Trace driven simulator.}
% \junchen{update this?}
In addition to the system implementation \cref{sec:system}, we also built a simulator to simulate the execution of training and inference jobs under varying resource constraints and workloads. The inputs to the simulator are execution traces from training and inference workloads with different configurations. 

To collect execution traces, we ran all configurations in our hyperparameter space on the 10 retraining windows for every video stream in the Waymo and Cityscapes datasets. For each training job execution in a retraining window, we log the training-accuracy progression over GPU-time. Once the model is trained, we also log its test accuracy over the future retraining windows to get the accuracy in future windows if it was not retrained. This builds an exhaustive trace set that allows us to simulate custom scheduling policies, modify the execution order, simulate resource sharing and allocation. All profiling and trace collection was done on a testbed with Nvidia RTX 2080 and Intel Xeon E-2226G CPU.

% Talk about the assumptions - inference accuracy min GPU, linear scaling etc

\textbf{Hyperparameters.}
For each training job, we create a fixed set of configurations by varying the following hyperparameters - number of epochs to train, batch size, number of neurons in the last layer, number of layers to retrain, and the fraction of data between retraining windows to be used for retraining. We then selected combinations of these hyperparameters to create a diversity in the resource-accuracy profiles of the configurations. 

\mypara{Performance metrics}
\junchen{tbd: accuracy, throughput (\# of streams) under given \# of gpus}

\textbf{Baselines.}
We compare the thief scheduler against a weighted {Fair Scheduler} \cite{fair-1, fair-2, videostorm}, which allocates equal resources to all video streams and within a video stream, allocates resources to training and inference proportional to the weight set as the \lstinline{inference_weight} parameter to scheduler. A higher \lstinline{inference_weight} implies a higher resource allocation to inference and a reduced allocation to training jobs. To pick retraining hyperparameters, the fair scheduler employs the common heuristic of highest-accuracy first. 

%We compare against two baselines. First is \textit{No-retraining}, which does not ever retrain the model and thus allocates resources only to inference. Second is \textit{Fair Scheduler} \cite{fair-1, fair-2, videostorm} which allocates equal resources to all video streams and within a video stream, allocates equal resources to both, training and inference. To pick retraining hyperparameters, the fair scheduler employs the common heuristic of highest-accuracy first. 
% Why are these good baselines?

% \textbf{Metrics.}
% % More:
% Our most used metric is Inference Accuracy over time, as described in \S\ref{subsec:formulation}. We also use the number of GPUs provisioned at the edge server as a measure of cost.


% \junchen{

% 6.2 Overall improvement

% - accuracy vs. gpus (fix \# of videos)

% - streams vs. gpus (fix accuracy)

% - accuracy vs. streams (fix \# of gpus)

% - alternative architectures



% 6.3 Understanding Ekya improvements

% - ablation analysis

% - per-stream gains

% - temporal behaviors



% 6.4 Microbenchmarking

% - estimation accuracy of microprofiling

% - impact of microprofiling erros

% - delay of thief scheduler

% - impact of scheduling granularity


% }

% overall improvement: 
% acc vs gpu
% mention the cloud baseline
\subsection{Overall improvements}

\begin{figure}
  \centering
%   \begin{subfigure}[t]{0.5\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{results/multicam/multicam_acc_vs_res_cityscapes.pdf} 
%     \caption{\small Cityscapes}
%     \label{fig:scalability-gpus-cityscapes}
%   \end{subfigure}
%   ~~~
%   \begin{subfigure}[t]{0.5\linewidth}
%     \centering
%     % \includegraphics[width=\linewidth]{figures/motivation/Class_Incrementality/class_distribution_change_sf_27.png}
%     \includegraphics[width=\linewidth]{results/multicam/multicam_acc_vs_res_waymo.pdf}
%      \caption{\small Waymo}
%     \label{fig:scalability-gpus-waymo}
%   \end{subfigure}
  \begin{subfigure}[t]{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{results/multicam/cityscapes_across_resources.pdf} 
    \caption{\small Cityscapes}
    \label{fig:scalability-gpus-cityscapes-golden}
  \end{subfigure}
  ~~~
  \begin{subfigure}[t]{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{results/multicam/waymo_across_resources.pdf} 
    \caption{\small Waymo}
    \label{fig:scalability-gpus-waymo-golden}
  \end{subfigure}
  \caption{\small \bf Multi-video performance: Our accuracy gain over baselines increases with more GPUs. \romil{Set x,y axis labels and use the custom size params for matplotlib formatting. Reviewer Q.: How do you partition 10 video streams over 8 GPUs?}}
  \label{fig:scalability-gpus}
\end{figure}

\mypara{Accuracy vs. provisioned resource}
Figure~\ref{fig:scalability-gpus} compares the performance of \name, average inference accuracy under same amount of total GPU resource, with the no-retraining baseline and the fair-scheduler baseline.
In each of the Waymo and Cityscapes traces, we randomly pick 10 video streams and run their inference concurrently through five retraining windows.
As we increase the number of provisioned GPUs, we see that \name consistently outperforms the best of the two baselines by a considerable margin
\romilc{xx}\%-\romilc{xx}\% points higher accuracy in Cityscapes and \romilc{xx}\%-\romilc{xx}\% points in Waymo.
Note that these gains in accuracy are achieved without increasing inference delay.
\name allocates resource to retraining only when the accuracy gain from retraining the model outweighs the temporary accuracy drop due to frame subsampling, which explains why \name outperforms the no-retraining baseline. 
Moreover, when \name allocates resource to retraining, it allocates minimum amount needed by the retraining to finish in time, thus outperforming the fair scheduler.
While accuracy gap between \name{} and the fair scheduler baseline decreases as more GPUs are provisioned, \name needs much less resources (upto $6.5\times$ less GPUs, Table \ref{tab::resource-savings-golden}) to achieve the maximum accuracy that fair scheduler attains with 8 GPUs.

%\name's gains over no-retrain baseline are more sizable in Waymo than Cityscapes, but its gains over the fair scheduler baseline are comparable in both traces. 
%This suggests that Waymo data is inherently more suitable for continuous retraining, but through more intelligent resource allocation, \name can always squeeze more juice from retraining than fair scheduler.



% \input{resource_table.tex}
\input{resource_table_golden_model.tex}
% gains per stream
\mypara{Performance per video stream}
Figure~\ref{fig:multicam-cities} shows the improvements {\em per video stream} of \name over the baselines, using the same 10 video streams as in Figure~\ref{fig:scalability-gpus} when 4 GPUs provisioned. 
Rather than trading accuracies among video streams, \name re-allocates resources in a way that improves accuracy for {\em all} of the video streams. 
That said, the accuracy gain varies, with gains being more considerable on video streams that have low accuracy without retraining (no-retraining).
This is because these video streams tend to have more dynamic scenes thus may benefit more from retraining.
This highlights a desirable behavior of \name that resource will more likely to be assigned where more accuracy gains are expected.
% \junchen{again, any insight as to what might cause the difference between the two traces?}



% % temporal variance
% \mypara{Timeseries of \name performance}
% Figure~\ref{fig:multicam-timeseries} zooms in on one of the video streams from Figure~\ref{fig:multicam-cities} (V\fillme) and presents the timeseries of performance of \name and the baselines over the five retraining windows. 
% This is one of the video streams that see a high accuracy gain over no-retraining. 
% The timeseries corroborates our intuition: when no-retraining accuracy is low (the \fillme-th retraining window), \name allocates resource to allow it to retrain its model which keeps the accuracy at a high value.

% \begin{figure}
% 	\includegraphics[width=0.4\textwidth]{results/multicam/multicam_taskwise_acc_zurich_4_cityscapes.pdf}
% 	\caption{\small \bf Timeseries of our performance vs. fair sharing. Again, adaptive resource sharing constantly outperforms fair sharing. \romil{Accuracy drops over time.}}
% 	\label{fig:multicam-timeseries}
% \end{figure}


% scalability: with more gpus, we can support more camera
\mypara{Scalability with more GPUs}
Next, we evaluate the scalability of \name's {\em throughput} as more GPUs are available.
We define throughput as the maximum number of video streams that can run concurrently on the GPUs while achieving a accuracy within a threshold of the maximum possible mean accuracy.
(This definition is common in practice, since applications usually require accuracy to be above a threshold for the inference to be usable.)
Figure~\ref{fig:scalability-gpu-vs-cam-thresholded} shows that \name's throughput grows almost linearly with more available GPUs, and at a rate \romilc{$2.3\times$} faster than the baseline of fair scheduler.
This suggests that \name can more easily scale to a large number of video sources than the baselines.

\begin{figure}
  \centering
%   \begin{subfigure}[t]{\linewidth}
%     \centering
%     \includegraphics[width=0.9\linewidth]{results/multicam/multicam_individual_stream_acc_cityscapes.pdf} 
%     \caption{\small Cityscapes Human Label}
%     %\label{fig:multicam-cities-cityscapes}
%   \end{subfigure}
    \begin{subfigure}[t]{\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{results/multicam/cityscapes_across_cities.pdf} 
    %\caption{\small Cityscapes Golden Model}
    %\label{fig:multicam-cities-cityscapes}
  \end{subfigure}
%   ~~~
%   \begin{subfigure}[t]{0.5\linewidth}
%     \centering
%     % \includegraphics[width=\linewidth]{figures/motivation/Class_Incrementality/class_distribution_change_sf_27.png}
%     \includegraphics[width=\linewidth]{results/multicam/multicam_individual_stream_acc_waymo.pdf}
%      \caption{\small Waymo}
%     \label{fig:multicam-cities-waymo}
%   \end{subfigure}
  \caption{\bf\small Multi-video performance: Ours (with continuous retraining) vs. Fair Share Scheduler. Compared across cities, we do consistently better. Some cities see bigger gains than others, which are thus prioritized by \name{}.}
  \label{fig:multicam-cities}
\end{figure}


Figure \ref{fig:scalability-fixedGPUs-accuracy} evaluates the throughput-accuracy tradeoff made by \name{} with a fixed number of resources. To minimize the accuracy variations between cities, we add video streams by replicating a fixed video stream from the Cityscapes dataset. 
With only a single GPU, increasing the number of video streams forces \name{} to gradually reduce resource allocation to retraining in favour of keeping of a high inference accuracy by allocating all resources to inference. The fair scheduler is unaware of the resource cost of retraining, and diverts GPU cycles from inference, resulting a lower inference accuracy.

\begin{figure}
 	%\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/single-tradeoffs.pdf}
 	\includegraphics[width=\linewidth]{results/scalability/scalability_GPUs_cams_cityscapes.pdf}
	\caption{\small \bf Throughput measured as number of video streams that can be concurrently supported for different resource sizes subject to accuracy thresholds.
	%The accuracy threshold is a multiplicative factor of the maximum achievable mean accuracy for a workload given $\infty$ resources.
	}
	\label{fig:scalability-gpu-vs-cam-thresholded}
\end{figure}

% SIGCOMM Results:
% \begin{figure}
%  	%\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/single-tradeoffs.pdf}
%  	\includegraphics[width=\linewidth]{results/scalability/scalability_cams_fixedGPUs_cityscapes.pdf}
% 	\caption{\small \bf Effect of adding more video streams on accuracy for different schedulers. When insufficient resources are provisioned, \name{} gracefully degrades to the No-retrain baseline, while the retraining decisions made by the fair scheduler reduce the mean inference accuracy.}
% 	\label{fig:scalability-fixedGPUs-accuracy}
% \end{figure}
\begin{figure}
 	%\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/single-tradeoffs.pdf}
 	\includegraphics[width=\linewidth]{results/scalability/scalability_cams_fixedGPUs_cityscapes_golden_model.pdf}
	\caption{\small \bf Using golden model. Effect of adding more video streams on accuracy for different schedulers. When insufficient resources are provisioned, \name{} gracefully degrades to the No-retrain baseline, while the retraining decisions made by the fair scheduler reduce the mean inference accuracy.}
	\label{fig:scalability-fixedGPUs-accuracy}
\end{figure}


% per video. even if one video, gains are impressive
\mypara{Gains with single video stream}
Figure~\ref{fig:singlecam-cities} presents the same analysis of Figure~\ref{fig:scalability-gpus} but with only one video stream using the resources.
Across these video streams (and many others but not shown), we see that \name consistently outperforms the baselines by dynamically deciding when to retrain the model as well as the resource balance between retraining and inference.
As in Figure~\ref{fig:multicam-cities}, we see the gains vary considerably across video streams, which again highlights that some video streams can inherently benefit more from retraining.% their models.

% \begin{figure}
%   \centering
%   \begin{subfigure}[t]{\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{results/singlecam/singlecam_acc_vs_cost_cityscapes.pdf} 
%     \caption{\small Cityscapes}
%     \label{fig:singlecam-cities-cityscapes}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[t]{\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{results/singlecam/singlecam_acc_vs_cost_waymo.pdf}
%     \caption{\small Waymo}
%     \label{fig:singlecam-cities-waymo}
%   \end{subfigure}
%   \caption{\bf\small Single-video performance - different videos have different payoffs for retraining.}% In \ref{fig:singlecam-cities-cityscapes}, V2 demonstrates large benefits to retraining compared to V4.}
%   \label{fig:singlecam-cities}
% \end{figure}

\begin{figure}
  \centering
  \begin{subfigure}[t]{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{results/singlecam/singlecam_acc_vs_cost_golden_cityscapes.pdf} 
    \caption{\small Cityscapes}
    \label{fig:singlecam-cities-cityscapes-golden}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{results/singlecam/singlecam_acc_vs_cost_golden_waymo.pdf}
    \caption{\small Waymo}
    \label{fig:singlecam-cities-waymo-golden}
  \end{subfigure}
  \caption{\bf\small Single-video performance - different videos have different payoffs for retraining.}% In \ref{fig:singlecam-cities-cityscapes}, V2 demonstrates large benefits to retraining compared to V4.}
  \label{fig:singlecam-cities}
\end{figure}


\subsection{Comparison with alternative designs}
\label{subsec:eval-alternate}

Next, we evaluate two alternative designs for continuous retraining---(1) re-using a retrained model from a history window that shares class distribution (instead of retraining the model again) and (2) offloading the retraining to the cloud.

\mypara{Advantage over re-using cached models}
Reusing a cached model from history is tempting as it avoids the cost of model retraining. 
%Figure~\ref{fig:history-vs-current} compares 
We compare the accuracy of retraining the model on the current window (\name) with the accuracy of re-using the model from a history window in which the class distribution is close to the distribution in the current window (Euclidean distance $\leq 0.2$; \S\ref{sec:profiling}). Here we use ResNet18 as the model and Waymo as the trace.
%The graph, however, shows 
We observe that 
the accuracy is much lower by re-using the model from history, even when the history window share a similar class distribution. At median, the difference in accuracy is 11\% with the $90^\text{th}$ percentile and maximum divergence in accuracies being as high as $38\%$ and $51\%$. 
This confirms our intuition in \S\ref{sec:profiling} that although sharing a similar class distribution is indicative of the difficulty of retraining, it does not mean the model can be directly reused from any window with similar class distribution.


%\begin{figure}[t!]
%\centering
%\includegraphics[width=0.6\columnwidth]{figures/eval_placeholders/history-trained-vs-retrained-cdf.pdf}
%\vspace{-0.2cm}
%\caption{\bf\small Gap between accuracy of the model retrained in the current and accuracy of re-using a model retrained in a history window that share similar class distribution.
%\vspace{-0.2cm}}
%\label{fig:history-vs-current}
%\end{figure}


\mypara{Advantage over a cloud-based solution}
Retraining could be offloaded to the cloud so the edge servers can focus on inference, but on a closer look such a cloud-based solution will even negate the benefit of retraining the model, because of the expensive communication delay from uploading training data to the cloud and downloading retrained models). 

%It is fundamentally challenging to run continuous learning across the edge-cloud because of network constraints.

% Math sheet new - https://docs.google.com/spreadsheets/d/1-WDeFmQwHy0sEpxL9f6QcbMKt1DVPaX6ODjMwDbb3IY/edit#gid=0
For instance, consider a setup serving 5 video streams in parallel with a retraining window size of 400 seconds. For a bit rate of 8 Mbps \cite{bitrate} and assuming a 10\% subsampling, it amounts to 320 Mb of training data being generated per camera in every retraining window. This retraining data must be uploaded to cloud and a model must be retrained and fetched back to the edge. Uploading 320 Mb over an average cellular uplink of 5.1 Mbps \cite{opensignal_2018} for 5 cameras results in a total upload time of 313 seconds. A model checkpoint of ResNet18 is 398 Mb, downloading which would take 23 seconds per camera on a downlink of 17.3 Mbps \cite{opensignal_2018}, or a total of 115 seconds for 5 cameras. The total network transfer cost is 428 seconds, which exceeds the retraining window size of 400 seconds. 

% Mention do we have to send everything to the cloud.

% examples where the drop is higher
Even on provisioning double the bandwidth (which entails an expensive change of the network link from cellular to cable), retraining on the cloud does not yield a higher accuracy in our simulator. We extend our simulator to simulate the network delays and assume that the the cloud offers a speed up of $10\times$ and has infinite parallel resources. Even then, the cloud \romilc{RTT} takes about 216 seconds and yields a mean inference accuracy of 81.8\%. In contrast, retraining at the edge completes in 125 seconds, leaving more time to take advantage of the retraining model, and results in an inference accuracy of 83.75\%.

% Show the calculation
% Mention the cost
% Varying network connections
Achieving the same accuracy in our simulations required increasing the downlink and uplink bandwidth by $3\times$ and still operates under the assumption that the cloud can provision parallel resources instantly, which can be expensive.

% Math sheet- https://docs.google.com/spreadsheets/d/1z4Zui8Qmg4iH-_yQKu7p0EZtXOlj_-ogKIW9mbf-Tpo/edit#gid=179811194

% For instance, each retraining window in the Waymo dataset accumulates about 1760 Mb of data every 20 seconds, resulting in a 88 Mb/s bitrate. Assuming a 10\% sub-sampling rate for retraining and a retraining window of 200 seconds (as in all our experiments), a total of 1760 Mb  of training data must be sent to the cloud. With an uplink of 5.1 Mb/s \cite{opensignal_2018}, just uploading the training data would take 345 seconds. Moreover, the updated model weights need to be downloaded from the cloud, which is 360 Mb in size. With a downlink throughput of 17.3 Mb/s \cite{opensignal_2018} (cellular connection), that adds another 20 seconds. Combined, this results in nearly 365s to get the retrained model, which far exceeds the retraining window size of 5 minutes (note that we have ignored the time to run the training in the cloud). Since even the sub-sampled video bitrate exceeds the limited bandwidths at the edge, this analysis applies for all retraining window sizes.


% \junchen{i still feel this should be in motivation section, no?}

\subsection{Sensitivity analysis}
\label{subsec:sensitivity-eval}

% \begin{figure} [t!]
%  	%\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/single-tradeoffs.pdf}
%  	\includegraphics[width=\linewidth]{results/ablation_waymo.pdf}
% 	\caption{\small \bf {\name} factor analysis by removing  dynamic resource allocation and reducing the hyperparameter space.}
% 	\label{fig:factor-analysis}
% \end{figure}

\begin{figure} [t!]
 	%\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/single-tradeoffs.pdf}
 	\includegraphics[width=\linewidth]{results/ablation_cityscapes_golden.pdf}
	\caption{\small \bf {\name} factor analysis by removing  dynamic resource allocation and reducing the hyperparameter space.}
	\label{fig:factor-analysis}
\end{figure}

% improvement breakdown
\mypara{Factor analysis}
To understand the contribution of each part of \name, we run a factor analysis on the same setting as Figure~\ref{fig:scalability-gpus} (10 video streams with 4 GPUs provisioned). We construct two schedulers from {\name}. \emph{Ekya-NoRes}, which removes the smart resource allocation in \name. \emph{Ekya-NoRes-NoEp} removes resource allocation and additionally fixes the number of epochs a model is trained to the maximum value, effectively removing it from the configuration space. We chose this hyperparameter for removal because it creates the largest diversity in the resource-accuracy profiles of configurations. 

As observed in Figure \ref{fig:factor-analysis}, the diversity in configurations and their careful selection has a large contribution to \name{}'s gains in accuracy when fewer resources are provisioned, which reduces as more resources are made available. This is because with more resources, even expensive configurations become feasible, thus configuration selection matters less. The smart resource allocation mechanism in {\name} has a nearly consistent contribution to \name{}'s performance.

%We note that the accuracy of \emph{Ekya-NoRes-NoEp} is lower than \emph{No-retrain} when 1 GPU is provisioned because resource reallocation is removed, and thus it always allocates resources to retraining. It just so happens that there are no good configurations to pick from once the epochs hyperparameter is removed, and thus the accuracy is lesser than \emph{No-retrain}.



% sensivity to accuracy errors
\mypara{Sensitivity to accuracy estimation errors}
\romil{Add paragraph and plot on accuracy of microprofiling.} %Resource consumption and accuracy of accuracy estimation. E
We now test the impact of errors in accuracy profiles (\S\ref{subsec:profiling}) on \name's performance gains.
To control the amount of errors, we add a controlled Gaussian noise on top of the real retraining accuracy as the predictions when the profiler is queried. 
Figure~\ref{fig:sensitivity-accuracy-error} shows that with upto 20\% errors in the profiler prediction, the maximum accuracy drop is 3\% points. When a 50\% profiling error is introduced, the accuracy drop is 7.9\% points. Such a large profiling error makes \name{} worse than the no-retrain baseline, but still better than fair scheduling.

\begin{figure}
	\includegraphics[width=\linewidth]{results/sensitivity/sensitivity_profileerrors_cityscapes.pdf}
	\caption{\small \bf Adding a controlled error $\epsilon$ to the accuracy prediction -  \name{}'s performance degrades, but only marginally.}
	\label{fig:sensitivity-accuracy-error}
\end{figure}

% Two subfigure plot for sensitivity 
% \begin{figure}
%   \centering
%   \begin{subfigure}[t]{0.5\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{results/sensitivity/sensitivity_profileerrors_cityscapes.pdf} 
% 	\caption{\small \bf Adding errors to the profiler.}
%     \label{fig:sensitivity-accuracy-error}
%   \end{subfigure}
%   ~~~
%   \begin{subfigure}[t]{0.5\linewidth}
%     \centering
%     % \includegraphics[width=\linewidth]{figures/motivation/Class_Incrementality/class_distribution_change_sf_27.png}
%     \includegraphics[width=\linewidth]{results/sensitivity/sensitivity_delta_acc_runtime_cityscapes_48gpu.pdf}
%      \caption{\small Effect of stealing parameter $\delta$ on the thief scheduler.}
%     \label{fig:sensitivity-delta}
%   \end{subfigure}
%   \caption{\small \bf Sensitivity Analysis Results.}
%   \label{fig:sensitivity-group}
% \end{figure}

% sensitivity to granularity
\mypara{Sensitivity to scheduling granularity} \ga{Change $\delta$ to $\Delta$ in the graphs and text.}
Finally, we show the sensitivity of \name to the allocation quantum $\delta$ (Algorithm \ref{algo:thief_sched}), which controls the runtime of the scheduling algorithm on the one hand and the result of the resource allocation on the other.
Figure~\ref{fig:sensitivity-delta} illustrates this tradeoff with the same setting as Figure~\ref{fig:scalability-gpus} (10 video streams with 4 or 8 GPUs provisioned).
Between $\delta=0.1$ and 1.0, higher $\delta$ reduces the runtime of the scheduler by 4$\times$, but the accuracy gain is severely affected. 
One should pick a higher $\delta$ only when the scheduler is relatively slow compared to a retraining window; otherwise, a low value of $\delta$ (fine-grained scheduling) is preferable.

\begin{figure}
  \centering
  \begin{subfigure}[t]{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{results/sensitivity/sensitivity_delta_acc_runtime_cityscapes_48gpu.pdf}
  \end{subfigure}
  \caption{\small \bf Effect of the $\delta$ parameter on the thief scheduler. Larger values decrease the accuracy but are faster to compute.}
  \label{fig:sensitivity-delta}
\end{figure}

\subsection{System Implementation}
\romil{WIP}
\romil{Move this up in the implementaiton section and start with this result.}
The Ekya implementation is an end-to-end system which can ingest video streams and distribute retraining and inference jobs over a pool of shared GPU resources. We ran this implementation on our Edge test-bed \ref{machine-specs}. The load on the system was varied by changing the number of video streams that must be processed in parallel on the same pool of resources. \cref{fig:sysimpl-result} illustrates the performance of Ekya comapred against the fair scheduler for Cityscapes and Waymo datasets. Ekya offers a consistently higher accuracy than the fair baseline (by upto 8\% points) and Ekya can achieve the same accuracy as the fair scheduler, but support $2\times$ the number of video streams in parallel on the same set of resources.

Ekya's performance is affected by the runtime efficiency of it's scheduler. The thief scheduler's search over the resource-configuration space \ref{algo:thief_sched} can be computationally expensive, but relative to retraining window size, it is a small cost. As shown in \Cref{fig:sensitivity-schedlatency}, the t  hief scheduler computes a resource allocation for a retraining window of 200 seconds even when multiple GPUs must be allocated.

\begin{figure}
  \centering
  \begin{subfigure}[t]{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{results/sensitivity/scheduler_resourcetime.pdf}
  \end{subfigure}
  \caption{\small \bf Thief scheduler latency for scheduling 10 video streams with varying available resource quantities and retraining period durations. The scheduler latency is a tiny fraction compared to the duration of the retraining period.  }
  \label{fig:sensitivity-schedlatency}
\end{figure}


\begin{figure}
  \centering
  \begin{subfigure}[t]{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{results/sys_impl/multicam_acc_vs_res_sysimpl_cityscapes.pdf} 
    \caption{\small Cityscapes}
    \label{fig:sysimpl-result-cityscapes}
  \end{subfigure}
  ~~~
  \begin{subfigure}[t]{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{results/sys_impl/sysimpl_varyingcities_waymo.pdf} 
    \caption{\small Waymo}
    \label{fig:sysimpl-result-waymo}
  \end{subfigure}
  \caption{\small \bf End-to-end accuracy on the system implementation on 1 GPU with varying number of cities.}
  \label{fig:sysimpl-result}
\end{figure}

==> evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We evaluate \name{} on two datasets, Waymo and Cityscapes. The main results are:

\begin{itemize}
    \item With multiple cameras sharing the same resources on an edge server, \name{} achieves upto 31.2\% points higher accuracy. Attaining the same accuracy with existing fair scheduling techniques would require upto $4.3\times$ more resources.
    \item With reduced resource provisioning, Ekya's performance gracefully degrades to the basline with no retraining by evaluating the cost of retraining on inference accuracy. 
\end{itemize}

\subsection{Methodology}
\label{subsec:eval-setup}

\noindent\textbf{Datasets.} For our evaluation, we use the Waymo Open\cite{waymo} and Cityscapes\cite{cityscapes} datasets, two popular video datasets containing dashcam footage of cars driving through cities in the US and Europe. Cityscapes has \romilc{xx} video streams (a total of \romilc{xx} hours of videos) while Waymo Open has \romilc{xx} video streams (a total of \romilc{xx} hours of videos)

The workload in cityscapes is constructed by treating each city's video as an independent video stream feeding into Ekya for inference and retraining. The workload in Waymo Open is constructed by creating video streams by concatenating segments from the dataset \romil{Zhengxu can add more here}. These workloads are representative of independent video-streams with local variations which necessitate retraining for their specific data-distributions.

\noindent\textbf{Trace driven simulator.}
To evaluate Ekya, we built a simulator to emulates the execution of training and inference jobs under varying resource constraints by collecting traces of accuracy-resource profiles of different configurations offline. This simulator allows custom scheduling policies to be plugged in and modify the run order and resource allocation for different jobs.
% Talk about the assumptions - inference accuracy min GPU, linear scaling etc

\textbf{Hyperparameters.}
For each training job, we create a fixed set of configurations by varying the following hyperparameters - \romilc{List and describe what each of them is.}. Combinations of these hyperparameters are carefully chosen to create a rich diversity in the resource-accuracy profiles of the configurations. 

\textbf{Baselines.}
We compare against two baselines. First is \textit{No-retraining}, which does not ever retrain the model and thus allocates resources only to inference. Second is \textit{Fair Scheduler}\cite{fairsched} which allocates equal resources to all video streams and within a video stream, allocates equal resources to both, training and inference.
% Why are these good baselines?

\textbf{Metrics.}
Our most used metric is Inference Accuracy over time, as described in \S\ref{subsec:formulation}. We also use the number of GPUs provisioned at the edge server as a measure of cost.

\subsection{End-to-end improvement}
\label{subsec:e2e-improvement}

In this section, we evaluate the end-to-end performance of \name{} on our trace simulator. For each of the Waymo and Cityscapes datasets, we run 10 video streams concurrently on Ekya through 5 retraining windows. Each window is 100 seconds long.

Figure \ref{fig:scalability-gpus} compares the performance of \name{} with the baselines when different different quantities of resources are provisioned at the edge server. Compared to the fair scheduler, \name{} achieves upto $17.8\%$ points higher accuracy on the Cityscapes dataset and upto $31.2\%$ \romil{This is the max() number} points higher accuracy on the Waymo dataset. 

While the percentage point gap between \name{} and the fair scheduler baseline decreases as more GPUs are provisioned, the marginal resource-cost of every percentage point increases as the accuracy increases. Table \ref{tab:resource-savings} demonstrates the resource cost of achieving a fixed accuracy across different video streams. A fair scheduler requires upto $4.3\times$ GPUs compared to \name{} to get the same accuracy and this is a best-case estimate, assuming linear scaling of training throughput with GPUs allocated.
% Formulate this as resource saving

% Per city
At a macro level, \name{} ensures that each video stream is strictly better off than not retraining despite non-uniform resource allocation. Figure \ref{fig:multicam-cities} shows the mean inference accuracy for each video stream. \name{} outperforms both baselines, fair allocation and no-retrain. All video streams do not benefit proportionally from retraining - the \name{} profiler is cognizant of this fact and prioritizes resource allocation for video streams which promise a higher accuracy.

%TODO: Add multi camera results - Model this as throughput - how many streams you can support to get the same accuracy.
\romil{TODO: Varying num of cameras}

% Time series - this seems like a very specific example - remove if unnecessary; Show an example where different resources are allocated
Further, Figure \ref{fig:multicam-timeseries} compares the inference accuracy of the V3 video stream from the Cityscapes dataset when 4 GPUs are provisioned. At training tasks 1, 3 and 4, retraining with a fair scheduler results in similar or lower accuracies compared to not retraining. However, \name{} is able to retrain the model and boost the inference accuracy without any degradation. 



% \begin{figure}[h!]
% 	\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/sharing-tradeoffs.pdf}
% 	\caption{\small \bf Multiple video streams sharing an edge cluster: Ours (with adaptive sharing) vs. ours (with fair sharing) vs. various baseline DNNs (without retraining). Our adaptive resource sharing scheme outperforms fair sharing because it is aware of the heterogeneous utility of resource to improve accuracy by different video streams.}
% 	\label{fig:sharing-tradeoffs}
% \end{figure}

% \begin{figure}[h!]
% 	\includegraphics[width=0.4\textwidth]{results/schedcompare_10cams.pdf}
% 	\caption{\small \bf Our performance gain over baselines increases with more GPUs. \romil{Instead of just mean over cameras, consider putting error bars at every marker}}
% 	\label{fig:scalability-gpus}
% \end{figure}



\begin{figure}
  \centering
  \begin{subfigure}[t]{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{results/multicam/multicam_acc_vs_res_cityscapes.pdf} 
    \caption{\small Cityscapes}
    \label{fig:scalability-gpus-cityscapes}
  \end{subfigure}
  ~~~
  \begin{subfigure}[t]{0.5\linewidth}
    \centering
    % \includegraphics[width=\linewidth]{figures/motivation/Class_Incrementality/class_distribution_change_sf_27.png}
    \includegraphics[width=\linewidth]{results/multicam/multicam_acc_vs_res_waymo.pdf}
     \caption{\small Waymo}
    \label{fig:scalability-gpus-waymo}
  \end{subfigure}
  \caption{\small \bf Our performance gain over baselines increases with more GPUs. \romil{Instead of just mean over cameras, consider putting error bars at every marker}}
  \label{fig:scalability-gpus}
\end{figure}

% \begin{figure}
% 	\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/scalability-cameras.pdf}
% 	\caption{\small \bf Our performance gain over baselines increases with more GPUs. \romil{Instead of just mean over cameras, consider putting error bars at every marker}}
% 	\label{fig:scalability-cameras}
% \end{figure}


\begin{figure}
  \centering
  \begin{subfigure}[t]{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{results/multicam/multicam_individual_stream_acc_cityscapes.pdf} 
    \caption{\small Cityscapes}
    \label{fig:multicam-cities-cityscapes}
  \end{subfigure}
  ~~~
  \begin{subfigure}[t]{0.5\linewidth}
    \centering
    % \includegraphics[width=\linewidth]{figures/motivation/Class_Incrementality/class_distribution_change_sf_27.png}
    \includegraphics[width=\linewidth]{results/multicam/multicam_individual_stream_acc_waymo.pdf}
     \caption{\small Waymo}
    \label{fig:multicam-cities-waymo}
  \end{subfigure}
  \caption{\bf\small Multi-video performance: Ours (with continuous retraining) vs. Fair Share Scheduler. Compared across cities, we do consistently better. Some cities see bigger gains, some see smaller.}
  \label{fig:multicam-cities}
\end{figure}

% \begin{figure}[h!]
%  	%\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/single-tradeoffs.pdf}
%  	\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/singlecam_e2e.png}
% 	\caption{\small \bf Multi-video performance: Ours (with continuous retraining) vs. Fair Share Scheduler. Compared across cities, we do consistently better. Some cities see bigger gains, some see smaller.}
% 	\label{fig:multi-acrosscities}
% \end{figure}

\begin{figure}
	\includegraphics[width=0.4\textwidth]{results/multicam/multicam_taskwise_acc_zurich_4_cityscapes.pdf}
	\caption{\small \bf Timeseries of our performance vs. fair sharing. Again, adaptive resource sharing constantly outperforms fair sharing. \romil{Accuracy drops over time.}}
	\label{fig:multicam-timeseries}
\end{figure}


\begin{table}[]
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Video\\ Stream\end{tabular}} & \multirow{2}{*}{Accuracy} & \multicolumn{2}{c|}{GPUs Required} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Resource\\ Savings\end{tabular}} \\ \cline{3-4}
                                                                        &                           & Ekya        & Fair Scheduler       &                                                                             \\ \hline
V0                                                                      & 76.6\%                    & 4           & 13.4                 & $3.3\times$                                                                 \\ \hline
V1                                                                      & 91.5\%                    & 4           & 4.4                  & $1.1\times$                                                                 \\ \hline
V2                                                                      & 78.1\%                    & 4           & 11.2                 & $2.8\times$                                                                 \\ \hline
V3                                                                      & 68.5\%                    & 4           & 14.9                 & $3.7\times$                                                                 \\ \hline
V4                                                                      & 66.9\%                    & 4           & 17.2                 & $4.3\times$                                                                 \\ \hline
V5                                                                      & 81\%                      & 4           & 6.4                  & $1.6\times$                                                                 \\ \hline
V6                                                                      & 80.9\%                    & 4           & 9.4                  & $2.3\times$                                                                 \\ \hline
V7                                                                      & 76.8\%                    & 4           & 15.1                 & $3.7\times$                                                                 \\ \hline
V8                                                                      & 67.8\%                    & 4           & 14.2                 & $3.5\times$                                                                 \\ \hline
V9                                                                      & 67.9\%                    & 4           & 8.9                  & $2.2\times$                                                                 \\ \hline
\end{tabular}
\label{tab:resource-savings}
\caption{Resource savings for different cities in the cityscapes dataset.}
\end{table}

\subsection{Single video stream performance}
In this section, we evaluate the performance of \name{} on single video stream. In this setup, only one video stream is provided to \name{}, so it must only pick training configurations for one stream and allocate all resources between the training and inference of this stream. 

Figure \ref{fig:single-tradeoffs} highlights the accuracy-cost characteristic demonstrated by different schedulers for 10 video streams from the cityscapes dataset, where each stream is run independently and does not share resources. For a fixed resource cost, \name{} achieves a higher accuracy than both Fair scheduler and no-retrain.  In $V6$, the accuracy gain from retraining is minimal, thus \name{} chooses not to retrain, while the fair scheduler retrains and results in a lower mean inference accuracy.

\begin{figure*}
 	%\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/single-tradeoffs.pdf}
 	\includegraphics[width=\linewidth]{results/singlecam/singlecam_acc_vs_cost_cityscapes.pdf}
	\caption{\small \bf Single-video performance: Ours (with continuous retraining) vs. various baseline DNN configurations (without retraining). Retraining allows ours to achieve much better accuracy-cost tradeoffs.}
	\label{fig:single-tradeoffs}
\end{figure*}


% \begin{figure}[h!]
% 	\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/single-timeseries.pdf}
% 	\caption{\small \bf Performance of ours (with continuous retraining) vs. baseline (without retraining) over time. Ours constantly outperforms the baseline due to continuous retraining. \romil{I assume this is similar to Figure 1?}}
% 	\label{fig:single-timeseris}
% \end{figure}


% \begin{figure}[h!]
%  	%\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/single-tradeoffs.pdf}
%  	\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/singlecam_e2e.png}
% 	\caption{\small \bf Single-video performance: Ours (with continuous retraining) vs. Fair Share Scheduler. Compared across cities, we do consistently better.}
% 	\label{fig:single-acrosscities}
% \end{figure}

\subsection{Implementation results}

\subsection{Sensitivity analysis}
\begin{itemize}
    \item Sensitivity to $\delta$ resource allocation quantum. \romilc{Affects the speed of convergence}
    \item Sensitivity to errors in profiling \cref{fig:sensitivity-accuracy-error}
    \item Sensitivity to hyperparameter configurations - Remove some of the best hyperparameters. \romilc{Ablation - remove hyperparameters, remove scheudling}
\end{itemize}

\begin{figure}
	\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/sensitivity-accuracy-error.pdf}
	\caption{\small \bf We add a controlled amount of error to the accuracy prediction and our performance does degrade but only marginally. \romil{Pick 5 cities, horizontal graph}}
	\label{fig:sensitivity-accuracy-error}
\end{figure}


\begin{figure}
  \centering
  \begin{subfigure}[t]{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{results/sensitivity/sensitivity_delta_acc_runtime_cityscapes_48gpu.pdf}
  \end{subfigure}
%   \begin{subfigure}[t]{0.5\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{results/sensitivity/sensitivity_delta_cityscapes.pdf} 
%     \caption{\small Accuracy}
%     \label{fig:scalability-gpus-cityscapes}
%   \end{subfigure}
%   ~~~
%   \begin{subfigure}[t]{0.5\linewidth}
%     \centering
%     % \includegraphics[width=\linewidth]{figures/motivation/Class_Incrementality/class_distribution_change_sf_27.png}
%     \includegraphics[width=\linewidth]{results/sensitivity/sensitivity_delta_runtime_cityscapes.pdf}
%      \caption{\small Runtime}
%     \label{fig:scalability-gpus-waymo}
%   \end{subfigure}
  \caption{\small \bf Effect of the $\delta$ parameter on the thief scheduler. Larger values decrease the accuracy but are faster to compute.}
  \label{fig:sensitivity-delta}
\end{figure}

% \begin{figure}[h!]
% 	\includegraphics[width=0.4\textwidth]{figures/eval_placeholders/sensitivity-video-accuracy.pdf}
% 	\caption{\small \bf Improvement by videos: Accuracy comparison ours vs baseline on different videos (with given cost budget).}
% 	\label{fig:sensitivity-video-accuracy}
% \end{figure}

\subsection{Alternate design points}

\noindent{\bf Cloud retraining.}

\noindent{\bf Specialized pre-trained models.}

==> microprofiling.tex <==
\section{Accuracy estimation with Microprofiling}
\label{sec:profiling}


% problem statement

% solution's principle - subset of data and configs

% subset of dataw

% config extrapolation (num. of epochs)

% prune out bad configs

% result teaser

% golden labels

% history-based alternate solution 


% profiling problem definition 
As shown in Figure \ref{fig:sys-arch} and explained in \S\ref{sec:solution}, {\name} relies on estimated accuracies of the retraining configurations for its scheduling decisions for each retraining window. Specifically, at the beginning of each retraining window $w$, the thief scheduler requires the estimated accuracy of each configuration $\gamma_v$, denoted as $a_v^{(w,\gamma)}$. The resource demands of the retraining configurations scale well with the size of the training data, and thus they only need to be measured once.

% Profiling
Predicting the accuracy of a fully trained model is challenging because it is dependent on the input data and stochastic training process. The problem is further compounded by the diversity in training configurations, which makes the training process unpredictable. However, as we show below, it is possible to predict the accuracy of a model within \romil{xx\%} if an initial seed knowledge of the model's training behavior is known. 

We simplify the accuracy prediction problem by training each configuration for a short duration on a sub-sample of the data. This micro-profiling process produces an accuracy value for each configuration when trained for a short duration on a subsample of the data. With each configuration's microprofiled accuracy as an input to the training loss curve model from \cite{optimus}, we can produce accuracy estimates for different epochs\romil{Add optimus model here}.

\cref{fig:microprofiling-bench} illustrates the effectiveness of micro-profiling in predicting model accuracy. We microprofile 6 hyperparameter configurations by training them for 5 epochs on 10\% data from a retraining window in the Cityscapes dataset. The accuracies produced by microprofiling are then used to estimate the accuracies if the model was trained without subsampling for 10, 20 and 30 epochs respectively. For comparison, we also train the same configurations for 10, 20 and 30 epochs without subsampling, indicated by the dotted curves. We see that \romil{...}

\romil{Talk about microprofiling cost/accuracy tradeoff?}

% Traditional hyperparameter tuning
Note that this problem different from the traditional hyperparameter tuning\cite{hyperband, asha}. Hyperparameter tuning involves picking the best performing configurations from a pool of candidate configurations, and thus can be modelled as a best-arm identification problem in a multi-armed bandit setting. It is implemented in a similar manner where multiple configurations are run in parallel and pruned as time progresses. However, our goal is not identifying the configuration which would yield the highest accuracy. We need to identify the training cost-accuracy tradeoff for each configuration such that the thief scheduler can make a globally optimal decision across configurations and video streams. Thus it is necessary to micro-profile each configuration instead of pruning configurations at runtime. 

{\bf Training labels.} Note that for the current retraining window as well as for the historical windows, {\name} acquires ``ground-truth'' labels using a golden model -- a high-cost but high-accuracy model pre-trained on a large dataset -- consistent with prior work \cite{incremental-13, mullapudi2019, incremental-15, distribution-20}. In every retraining window, {\name} runs the golden model on the training data to generate labels for retraining. We use the ResNet152 model trained on the MS-COCO dataset as our golden model. The cost of running the golden model is typically small (measured to be under $3\%$ of the retraining cost, as per our experiments).
% \romil{Add experiment to justify that golden model outputs are indeed representative of the ground truth}

\begin{figure}
  \centering
  \begin{subfigure}[t]{\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{results/microprofiling_dummy.pdf}
  \end{subfigure}
  \caption{\bf\small Errors in accuracy prediction when using Microprofiling. Accuracy errors are higher when predicting for larger number of epochs, but still within xx\% of the true accuracy.}
  \label{fig:multicam-cities}
\end{figure}



==> overview.tex <==
\section{Overview of {\name}}
\label{sec:overview}

The primary purpose of {\name} is to help network administrators investigate reports of poor network performance, i.e., RTTs between the clients and the cloud locations being above the desired SLOs. {\name} attributes such {\em path-level} latency degradations to localize the faults at the {\em AS-granularity}. %An approach that we considered was to use network tomography to infer AS-level latencies from the path-level latencies, and find the faulty AS based on deviations from their normal latencies. However, even though network tomography is a well-studied field~\cite{tomography papers}, no practical solutions exist especially at the scale of the Internet. This is due to two main reasons: ($i$) the passively collected measurements have a highly skewed visibility of the paths between the {\azure} locations and the different client AS'es (\S\ref{section-2}), and ($ii$) the sheer scale of the potential number of bad AS-paths preclude a full-scale probing because of the substantial overheads (Figure~\ref{??}). 
%{\name}'s design uses the passively collected RTT measurements to get a coarse localization of the problem (\xref{sec:passive}), and then use as few active probes as possible to finely diagnose those latency degradations that affect the most users (\xref{sec:active}). 
%Thus, in our design on {\name}, we strive to accurately diagnose those latency degradations that affect the most users users but using as few active probes as possible. 
In this section, we explain the high-level intuitions behind our solution before elaborating on the details in \xref{sec:passive} and \xref{sec:active}. 

%In designing {\name}, thus, we have two high-level goals that are important in practice: ($a$) accurately diagnose those latency degradations that affect the most users users, and ($b$) use as few active probes as possible. {\name} meets the goals with two core techniques both built upon our operational experience. Here we first elaborate their intuitions before presenting the details in next few sections.

\subsection{Two-level blame assignment}
\label{subsec:two-level}

Modeling the paths between the cloud locations and client at the AS-granularity, as per traditional approaches \cite{castro2004network, zhang2004planetseer}, is problematic. First, the coverage of the measurements is skewed and therefore there are often not sufficient measurements to identify the contributions by each AS in the path. Second, modeling the graph at the AS granularity introduces ambiguities, e.g., a large AS like Comcast might have a problem along certain paths but not all. The impact of both these problems is compounded when paths in the Internet change.

Instead of modeling a path as a concatenation of AS'es, {\name} views each path in two granularities---a {\em coarse-grained} segmentation of the path into three segments of ``client'' (the client AS), ``cloud'' (the cloud AS), and ``middle'' (all AS'es between the cloud and the client), and then a {\em fine-grained} AS-level view  of only the ``middle'' segment. Correspondingly, {\name} localizes the fault in two steps. 
\begin{enumerate}
    \item Attribute the blame for latency degradation on one of the three coarse segments, using {\em only} ``passive'' data.
    \item If a fault is attributed to a middle segment, {\name} (optionally) moves to the ``active'' phase to trigger probes for AS-level fault localization. 
\end{enumerate} 
Note that modeling {\em each} path into three segments (albeit at a coarse granularity) allows {\name} to identify localized issues in an AS that occur only in that path (but not elsewhere in that AS, thus avoiding the ambiguities explained above). 

%The coarse-grained blame assignment at the segment level is inspired by the operational observation that most cases of inflated latency is typically attributable to a single segment among the ``client'', ``middle'' and ``cloud'' along the end-to-end path (\ga{Support analysis?}). For example, inflated latency between an {\azure} location and the client might be due to the middle segment or the client prefix but not due to moderate increases in both. Inspired by this observation, we propose a simple-yet-practical algorithm to uniquely attribute a fault to one bad segment. %We notice that the two-level blame assignment over a network topology  
%We notice that the coarse-grained blame assignment of {\name} can be viewed as a practical instantiation of network tomography over potentially correlated links (e.g.,~\cite{imc10}). \ga{Correlated? What does this mean?}
%though we do not make much idealized assumption as in boolean tomography.

\noindent{\bf Coarse Segmentation:} The three-way segmentation of each path into client, middle, and cloud segments is borne out of {\azure}'s operational requirements. Localizing the fault to the cloud or the client AS is already actionable. A {\em cloud-induced} latency degradation would directly lead to personnel being deployed for further investigation. When the problem lies with the {\em client} network (e.g., the client's ISP), the cloud operator typically cannot fix the problem other than informing the client about their ISP choices (e.g., \cite{youtube-interruptions}). Thus, our segmentation proved to be pragmatically beneficial and allowed for a phased deployment. Our coarse-grained fault localization solution based on passive measurements has been deployed in production since Nov 2017.  %While we considered other sophisticated ways to cluster the AS'es to produce a coarser graph, the simple segmentation along client, middle, and cloud segments proved to be a pragmatically beneficial choice.

%The three-way segmentation of each path into client, middle, and cloud segments is largely aligned with the types of remedial actions that follow the blame assignment. A {\em cloud-induced} latency degradation would fall under the direct control of cloud operators leading to tools and personnel being deployed for further investigation. When the problem lies with the {\em client} network (e.g., the client's ISP), the cloud operator typically cannot fix the problem other than informing the client about their ISP choices (e.g., \cite{youtube-interruptions}). If the problem is caused by any of the AS'es in the {\em middle}, then the mitigation techniques include switching egress peering points and communicating with the administrators of the problematic AS'es. (\ga{Then why do you want to go to AS-level?}) Thus, the coarse-grained localization already provides actionable information to network engineers on the nature of the problem, even before the fine-grained localization.
% More importantly, assigning the latency inflation at the granularity of ``cloud'', ``middle'', and ``client'' sometimes already provides actionable information to help engineers take remedial steps.
% Note that even if there are multiple bad segments, {\name} will always return one of them, i.e., no false positives.


\subsection{Impact-proportional budgeted probing}
\label{subsec:impact-proportional}

%{\name}'s characterization of the fault into cloud, middle, client segments is incomplete towards the goal of AS-level fault diagnosis as the ``middle'' segment may contain multiple AS'es. However, as explained earlier, the passive measurements are insufficient to do AS-level fault diagnosis because of the lack of coverage of all the paths (see \xref{section2} and \S\ref{subsec:problem}). 
%The two-level blame assignment is incomplete, as it is insufficient to only use the passive end-to-end measurements to uniquely localize a middle-segment fault to a specific link. This is because to distinguish two potential fault links, there must be a measurement path traversing one and only one of them~\cite{imc14}. Cloud providers often lack such measurement diversity in the middle segment.  Clients are more likely to be mapped to a single ``nearest'' cloud site than others, so it is hard to localize the faults near the clients as these downstream links always co-occur with the same upstream links (more details in \S\ref{subsec:formulation}).

%{\name} uses active probes (traceroutes) to compensate for the lack of path coverage. Since probing all the paths for full coverage is prohibitively expensive given the sheer number of paths, {\name} sets a {\em budget} on the active probes and allocates the probes to bad middle segments based on their expected {\em impact} on clients. For each bad middle segment, {\name} estimates {\em how many clients will be affected} and {\em for how long}, and prioritizes those that are expected to affect more clients for longer time. 
{\name} uses active probes (traceroutes) only for fine-grained localization of ``middle'' segment blames, as these segments may contain multiple AS'es. Since probing all the paths for full coverage is prohibitive given the sheer number of paths (172 million per day; \xref{subsec:active-eval}), {\name} sets a {\em budget} on the active probes and allocates the budget to probing bad middle segments based on their expected {\em impact} on clients (\xref{subsec:ip-vs-impact}), i.e., by estimating {\em how many clients will be affected} and {\em for how long}. %, and prioritizes those that are expected to affect more clients for longer time. 
{\name}'s budgeted probing is unique in two aspects compared to prior work (e.g.,~\cite{zhang2004planetseer, 35590, madhyastha2006iplane}).

Spatially, {\name} defines the importance of a segment in proportion to its impact on actual {\em number of clients}, rather than just the addresses in the IP block \cite{35590}. In {\azure}'s operations, large IP address blocks often have fewer active clients than smaller IP blocks, thus making it desirable to predict and prioritize issues affecting the most active clients.
%While the size of an IP block can sometimes indicate the number of users, in our context, large IP blocks may have proportionally less active clients of the cloud service than smaller IP blocks. 

Temporally, %the number of active clients in a middle segment does not necessarily correlate with the {\em timespan} for which latency degrades. By 
by {\em estimating} the timespan of each latency degradation, {\name} can focus on long-lived problems rather than fleeting problems that may end shortly after we probe it, thus wasting our limited budget for probing. Note that we do not need very precise estimate on the timespan of a problem because of the long tail distribution of problem durations (\xref{subsec:long-tail}). It would suffice if we only separate the few long-lived problems from the many short-lived problems.%, and as shown in \S??, this can be estimated by how long the problem has lasted thus far. 

\subsection{End-to-end workflow} 

{\name}'s workflow is as follows. RTT data is passively collected at the different cloud locations and sent to a central data analytics cluster. %A data analytics job is periodically scheduled to run to categorize all RTTs that are higher than the desired SLOs and assign blames at coarse-grained segments; \xref{sec:passive}. 
A data analytics job periodically makes coarse-grained blame assignments to all bad RTT instances; \xref{sec:passive}. 
These blame assignments trigger two sets of actions. The middle segment issues are ordered based on their impact and active probes are issued from the appropriate cloud servers for finer localization; \xref{sec:active}. All the latency inflations are prioritized based on their impact, and the top few are sent to network administrators for investigation (details in \S\ref{subsec:implementation}). 

%\junchen{%below is from the old 4.1. needs to be merged in sec 3 as current operational practices:
%The primary purpose of {\name} is to help network administrators investigate reports of poor network performance, specifically, the RTTs between the clients and the cloud locations that are above the desired SLOs. A key step in their investigations is identifying the {\em location} (at the granularity of an AS) that is the cause of the increased RTT. As described in \xref{sec:overview}, the result of the fault localization helps operators take a variety of different mitigating steps.
%\ga{Stitch into Intro.} Our conversations with the administrators of \azure revealed that, in the absence of problem localization, their current practice is to pick a handful of incidents of poor network performance from the last {\em day} (or from the last few hours), often in an ad hoc manner, and investigate these. This often results in investigating issues that are not directly fixable by the cloud operators (e.g., client ISP fault) as well as ignoring issues that are severe (e.g., cloud's fault with many affected clients). Moreover, this manual process tends to be slow, so much so that many faults get ``auto-resolved'' by the time the administrators get around to investigating them. Thus, the need for prioritizing incidents and investigating them closer to their occurrence (i.e., near real-time). }

==> profiling.tex <==
\section{Accuracy estimation for retraining configurations}
\label{sec:profiling}

% profiling problem definition 
As shown in Figure \ref{fig:sys-arch} and explained in \S\ref{sec:solution}, {\name} relies on estimated accuracies of the retraining configurations for its scheduling decisions for each retraining window. Specifically, at the beginning of each retraining window $w$, the thief scheduler requires the estimated accuracy of each configuration $\gamma_v$, denoted as $a_v^{(w,\gamma)}$. The resource demands of the retraining configurations scale well with the size of the training data, and thus they only need to be measured once.

% history vs. current window
We consider two broad approaches to estimating the accuracy, $a_v^{(w,\gamma)}$. The first approach is {\em online} where a ``profiler'' is executed on a sub-sample of the training data on all candidate configurations \cite{videostorm}. However, this approach is time-consuming and strains the already resource-constrained edge server. Instead, we use {\em history} and predict the accuracy using accuracy values from prior retraining windows.

% history; class distribution 
History-based profiling is widely used to optimize machine-learning systems (\eg~\cite{awstream,chameleon}). 
A natural approach is to predict $a_v^{(i,\gamma)}$ using a moving-window average over a history of $k$ retraining windows, $a_v^{(i-1,\gamma)},a_v^{(i-2,\gamma)},\dots,a_v^{(i-k,\gamma)}$ where $\gamma$ is the retraining configuration. The main drawback with this approach is that it mixes accuracy values from windows with different class distributions. A better approach, instead, is to use only those prior windows whose class distributions are similar to the current window. We use the Euclidean distance as our measure of similarity between class distributions. %It aggregates the accuracy values from similar history windows, grouped by individual configurations. 


%\begin{figure}[t!]
%\centering
%\includegraphics[width=0.8\columnwidth]{figures/eval_placeholders/cdf-profiler-error.png}
%\vspace{-0.2cm}
%\caption{\bf\small \name's profiler can predict the model accuracy after retraining with less error than the baseline of moving average over recent history windows.\zhengxu{pdf file added. change filename in tex when needed}\romil{We should pdf this}
%\vspace{-0.2cm}}
%\label{fig:profiler-error}
%\end{figure}


% insight
Given the inherent tradeoff between compressing models (for efficiency) and their generalizability (\S\ref{subsec:continuous}), the closer the distribution of classes is between two retraining windows, the similar the accuracies are of the models retrained in those windows. Our evaluations of the above simple predictor on the different video datasets from Cityscapes and Waymo (\S\ref{subsec:eval-setup}) show that our prediction (of accuracy) is nearly $10\%$ points better at the median (and $18\%$ points at the $90^\text{th}$ percentile).%; see Figure \ref{fig:profiler-error}.  
%The insight is that the accuracy of a retrained model depends more on difficulty of the data used to retrain the model. For instance, if the training data consist of only a handful of classes, the retrained model can be very high accurate since the data have low complexity. Otherwise, if the training data include tens of classes, the retrained model will tend to have slightly lower accuracy on each class, due to the inherent capacity/complexity tradeoff of cheap DNN models. In other words, if two retraining windows are comprised of similar distribution of classes, the retraining accuracies tend to similar. (Of course, there can be other metric of difficulty of the training data than class distribution, but we empirically found class distribution works well in our setting.)
% \gaa{We should stress that even if two windows have similar class distributions, it does not mean the retrained model from one window can be re-used in the other due to discrepancies in other aspects (camera lighting, angles of objects, etc; \S\ref{subsec:continuous-measurement}).}

We should stress that even if two windows have similar class distributions, it merely means the two windows are equivalent in their difficulty to reach high accuracy through retraining; it does {\em not} mean the retrained model from one window can be re-used in the other (as \S\ref{subsec:continuous-measurement} showed, other factors such as lighting and angles of objects may be considerably different between the two windows). We show the degraded accuracy of such a solution that caches and uses past models from windows with similar class distributions in \S\ref{subsec:eval-alternate}.
% due to discrepancies in other aspects (camera lighting, angles of objects, etc; \S\ref{subsec:continuous-measurement}).

% no history available 
When there is no retraining window in history with similar distributions for the configuration $\gamma$, {\name} resorts to the online approach. It retrains using $\gamma$ on a small fraction of the training data. The accuracy from these runs are provided to Algorithm \ref{algo:thief_sched}. \name seldom has to resort to the online approach since it looks sufficiently long back in history. 
%For instance, one can try several retraining configurations in parallel on a small subsample of the training data. In the case when there is no history window with similar class distribution that used the queried retraining configuration, by default \name will apply the configuration to retrain the model (if there is enough resource).
% exploration phase; exhaustive profiling to identify promising configurations 
To build a rich history, \name periodically opts for a randomly chosen configuration (from the Pareto boundary) in its retraining. Such an approach of ``exploration'' allows it to build a mapping between data distributions, configurations, and their accuracy values. 

{\bf Training labels.} Note that for the current retraining window as well as for the historical windows, {\name} acquires ``ground-truth'' labels using a golden model -- a high-cost but high-accuracy model pre-trained on a large dataset -- consistent with prior work \cite{incremental-13, mullapudi2019, incremental-15, distribution-20}. In every retraining window, {\name} runs the golden model on the training data to generate labels for retraining. We use the ResNet152 model trained on the MS-COCO dataset as our golden model. The cost of running the golden model is typically small (measured to be under $3\%$ of the retraining cost, as per our experiments).
% \romil{Add experiment to justify that golden model outputs are indeed representative of the ground truth}


% empirical numbers
%To show the effectiveness of our idea, Figure~\ref{fig:profiler-error} picks a retraining configuration (retraining last layer of ResNet18) and compares the prediction error of two strategies per Waymo retraining window: running average over recent four history windows (baseline) and average over windows with similar class distributions (\name's profiler).\footnote{Notice that this is an idealized assumption; \name will not have a measured accuracy of the same configuration in all history windows, but the fact that our method based on class distribution similarity uses less windows, so in practice, our prediction can be even more accurate than the baseline.} To identify retraining windows that have similar class distribution, we group the class distributions into 5 clusters which acount for 70\% of retraining windows. We see that \name has on average 10\% lower prediction errors (with more reduction on the high percentiles). We should stress that even if two windows have similar class distributions, it does not mean the retrained model from one window can be re-used in the other due to discrepancies in other aspects (camera lighting, angle, etc).



==> profiling_JJ.tex <==
\section{Resource-accuracy of retraining configurations}
\label{sec:profiling}


\name relies on accurate estimation of retraining accuracy to decide if the inference model needs to be retrained to cope with data drifts.
% goal
At the $i$-th retraining window, \name's profiler takes in as input a retraining configuration $\gamma\in \Gamma_v$ and returns the estimated accuracy, denoted as $a_v^{(i,\gamma)}$, if \name retrains the model using $\gamma$ now and tests the new model on the remaining portion in the current window.


% natural solution: recent history. not practical for two reasons (1) model is rarely retrained recently, and (2) even it's retrained, the scene will be quite different
A natural strawman is to predict $a_v^{(i,\gamma)}$ using {\em recent history}; \eg a moving-window average over a group of $k$ retraining windows, $a_v^{(i-1,\gamma)},a_v^{(i-2,\gamma)},\dots,a_v^{(i-k,\gamma)}$.
History-based profiling is widely used to optimize machine-learning systems when input data evolve gradually (\eg~\cite{awstream,chameleon}).
However, it may not work well in our setting for two reasons.
First, for the benefits of retraining to outweigh the cost, retraining will only happen intermittently, so the same video is unlikely to have experienced retraining with the same configuration in many of the recent retraining windows.
Second, if the retrain did happen in the last history windows and the model needs to be retrained in the current window, it suggests there has substantial data drift between now and the retraining window when the model was retrained, so the retraining accuracy at that history window may not be indicative to our current window.


% our solution: find history windows that have similar difficulty
Instead, we use history information from more history retraining windows (10s to 100s), but 
% in which the same configuration is used for more times. 
rather than averaging $a_v^{(j,\gamma)}$ over any window $j$, \name uses only the windows whose class distributions are similar to the current window. 
We assume the golden model is running at a low frequency so that it takes negligible resources but still maintain a rough estimate of the distribution of classes in each retraining window.


The insight is that the accuracy of a retrained model depends more on difficulty of the data used to retrain the model. 
For instance, if the training data consist of only a handful of classes, the retrained model can be very high accurate since the data have low complexity.
Otherwise, if the training data include tens of classes, the retrained model will tend to have slightly lower accuracy on each class, due to the inherent capacity/complexity tradeoff of cheap DNN models.
In other words, if two retraining windows are comprised of similar distribution of classes, the retraining accuracies tend to similar. (Of course, there can be other metric of difficulty of the training data than class distribution, but we empirically found class distribution works well in our setting.)
There are other refinements that can be integrated in \name.
For instance, one can try several retraining configurations in parallel on a small subsample of the training data. 
In the case when there is no history window with similar class distribution that used the queried retraining configuration, by default \name will apply the configuration to retrain the model (if there is enough resource).

% some empirical numbers
To show the effectiveness of our idea, Figure~\ref{fig:profiler-error} picks a retraining configuration (retraining last layer of ResNet18) and compares the prediction error of two strategies per Waymo retraining window: running average over recent four history windows (baseline) and average over windows with similar class distributions (\name's profiler).\footnote{Notice that this is an idealized assumption; \name will not have a measured accuracy of the same configuration in all history windows, but the fact that our method based on class distribution similarity uses less windows, so in practice, our prediction can be even more accurate than the baseline.}
To identify retraining windows that have similar class distribution, we group the class distributions into 5 clusters which acount for 70\% of retraining windows.
We see that \name has on average 10\% lower prediction errors (with more reduction on the high percentiles).
We should stress that even if two windows have similar class distributions, it does not mean the retrained model from one window can be re-used in the other due to discrepancies in other aspects (camera lighting, angle, etc).

\begin{figure}[t]
\centering
%\includegraphics[width=0.4\textwidth]{figs/junchen/video-market-new.pdf}
\includegraphics[width=0.3\textwidth]{figures/eval_placeholders/cdf-profiler-error.png}
\vspace{-0.2cm}
\caption{\name's profiler can predict the model accuracy after retraining with less error than the baseline of moving average over recent history windows.
\vspace{-0.2cm}}
\label{fig:profiler-error}
\end{figure}

==> resource_table.tex <==

\begin{table}[t]
\small
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Video\\ Stream\end{tabular}} & \multirow{2}{*}{Accuracy} & \multicolumn{2}{c|}{GPUs Required} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Resource\\ Savings\end{tabular}} \\ \cline{3-4}
                                                                        &                           & Ekya        & Fair Scheduler       &                                                                             \\ \hline
V0                                                                      & 76.6\%                    & 4           & 13.4                 & $3.3\times$                                                                 \\ \hline
V1                                                                      & 91.5\%                    & 4           & 4.9                  & $1.2\times$                                                                 \\ \hline
V2                                                                      & 78.1\%                    & 4           & 11.2                 & $2.8\times$                                                                 \\ \hline
V3                                                                      & 68.5\%                    & 4           & 14.9                 & $3.7\times$                                                                 \\ \hline
V4                                                                      & 66.9\%                    & 4           & 17.2                 & $4.3\times$                                                                 \\ \hline
V5                                                                      & 81\%                      & 4           & 6.4                  & $1.6\times$                                                                 \\ \hline
V6                                                                      & 80.9\%                    & 4           & 9.4                  & $2.3\times$                                                                 \\ \hline
V7                                                                      & 76.8\%                    & 4           & 15.1                 & $3.7\times$                                                                 \\ \hline
V8                                                                      & 67.8\%                    & 4           & 14.2                 & $3.5\times$                                                                 \\ \hline
V9                                                                      & 67.9\%                    & 4           & 8.9                  & $2.2\times$                                                                \\ \hline
\end{tabular}
\caption{\bf\small Resource savings for different cities in Cityscapes.}
\label{tab:resource-savings-final}
\end{table}

==> resource_table_golden_model.tex <==

\begin{table}[t]
\small
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Video\\ Stream\end{tabular}} & \multirow{2}{*}{Accuracy} & \multicolumn{2}{c|}{GPUs Required} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Resource\\ Savings\end{tabular}} \\ \cline{3-4}
                                                                        &                           & Ekya        & Fair Scheduler       &                                                                             \\ \hline
V0                                                                      & 75.6\%                    & 4           & 15.6                 & $3.9\times$                                                                 \\ \hline
V1                                                                      & 78.6\%                    & 4           & 10.0                  & $2.5\times$                                                                 \\ \hline
V2                                                                      & 76.5\%                    & 4           & 19.5                 & $4.9\times$                                                                 \\ \hline
V3                                                                      & 74.5\%                    & 4           & 17.4                 & $4.4\times$                                                                 \\ \hline
V4                                                                      & 75.1\%                    & 4           & 20.9                 & $5.2\times$                                                                 \\ \hline
V5                                                                      & 71.4\%                      & 4           & 25.8                  & $6.5\times$                                                                 \\ \hline
V6                                                                      & 79.5\%                    & 4           & 8.05                  & $2.0\times$                                                                 \\ \hline
V7                                                                      & 75.3\%                    & 4           & 21.8                 & $5.5\times$                                                                 \\ \hline
V8                                                                      & 75.0\%                    & 4           & 84.5                 & $21.1\times$                                                                 \\ \hline
V9                                                                      & 75.2\%                    & 4           & 177.8                  & $44.5\times$                                                                \\ \hline
\end{tabular}
\caption{\bf\small Resource savings for different cities in Cityscapes. \romil{We should write DNF for V7 V8 V9. \romil{This is a bit confusing because every row is not running independently - so this isn't  per resource saving. We should either get overall aggregate number here or run V0 repeatedly to get per video number.}}}
\label{tab:resource-savings-golden}
\end{table}

==> stuff.tex <==
% Resource util maps
\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/motivation/Scheduler/schedmot_res_eventual_best_cfgs.pdf}
    \caption{\small Naive, eventual best cfgs}
    \label{fig:schedmot-res-naive}
  \end{subfigure}  
%  ~~
%  \begin{subfigure}[t]{0.3\linewidth}
%    \centering
%    \includegraphics[width=\linewidth]{figures/motivation/Scheduler/schedmot_res_optimal_cfgs.pdf}
%    \caption{\small Optimal cfgs for retraining window}
%    \label{fig:schedmot-res-optimalcfg}
%  \end{subfigure}
  ~~
  \begin{subfigure}[t]{0.5\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/motivation/Scheduler/schedmot_res_prioritization_and_optimal_cfgs.pdf}
    \caption{\small Optimal cfgs with prioritization}
    \label{fig:schedmot-res-prioritization}
  \end{subfigure}
  ~~
  \caption{\bf\small Resource allocation maps for toy retraining schedules in Figure \ref{fig:schedmot}. (\ref{fig:schedmot-naive}) and (\ref{fig:schedmot-res-optimalcfg}) run a fair scheduler which evenly splits resources between the two cameras. (\ref{fig:schedmot-res-prioritization}) deprioritizes Camera B's inference task due because of its low accuracy, and instead focuses resources on retraining it. On the other hand, Camera A's inference job is already at an high accuracy, thus it deprioritizes it's retraining job until Camera B is retrained. \ga{Unused GPUs when retraining is not happening; can we fix it?}}
  \label{fig:schedmot-res}
\end{figure}


\subsection{Checkpointing Models}
\label{subsec:checkpoint}
In the process of retraining, the inference accuracy increases only when the model being retrained is loaded into the inference job's memory. This checkpointing has both, a benefit (the accuracy improvement is available faster, thus mean inference accuracy increases) and a cost (cost of checkpointing model and loading into memory). Thus, the frequency of checkpointing is a careful decision dependent on the expected gain in accuracy and the cost of checkpointing.  \romil{Add figure like Fig 5b, except with more frequent checkpointing to show smooth increase and overall higher accuracy.}

\textbf{How do we do checkpointing?} Ekya carefully evaluates the cost-benefit of checkpointing to arrive at the optimal checkpointing rate. The cost is defined as the amount of time it takes to checkpoint a model in memory and reload it into the inference model. The benefit of checkpointing is the higher accuracy that will available for the remainder of the retraining period.

\textbf{Measuring the cost ($\delta$): } The time taken to checkpoint a model and load it is dependent on the size of the model. While the model is being checkpointed, the model training must be halted \romilc{Should it?}. Since the model size and architecture does not change over retraining windows, it is possible to profile the checkpoint cost beforehand. In our experiments \romilc{TODO}, we found that checkpointing requires \romilc{xx} seconds and restoring requires \romilc{yy} seconds, creating a total cost of \romilc{$\delta$} seconds on the checkpointing 

\textbf{Measuring the benefit (accuracy improvement): } Consider a single video stream with a single retraining job and a single inference job. Let $\tau$ be the time taken by the retraining job to complete. At any time instant $t$ since the start of the retraining window, let the inference accuracy of the job be $a$. The remaining amount of time in the window can be calculated as $T-t$, where $T$ is the length of the retraining window and $A$ is the final retrained accuracy. Without checkpointing, the mean inference accuracy in the remainder retraining window is \romil{Change to integral}:

\[
    base\_acc = \frac{(\tau-t)*a + (T-\tau)*A}{T} 
\]

With checkpointing (\romilc{Figure xx}), \name{} must decide if at every timestep $t$ the model must be checkpointed. By checkpointing, the inference accuracy improves while the retraining is still running, but a checkpoint also increases the total train time by $\delta$. Assume the inference accuracy at start is $a$ and increases to $a^{*}$ Thus the inference accuracy if checkpointed at time $t$ is:  \romil{Careful, this is validation accuracy.. maybe include a validation->test acc conversion facor?}
\[
    acc = \frac{(\tau-t)*a^{*} + (T-\tau-\delta)*A}{T} 
\]

\textbf{Checkpointing Decision} Thus, models must be checkpointed only when $acc > base\_acc$, and this decision is evaluated at every time instant $t$. Whenever this statment is true at the current $t$, the model is checkpointed.


